CompartOS: CHERI Compartmentalization for Embedded Systems

Existing high-end embedded systems face frequent security attacks. Software compartmentalization is one technique to limit the attacks' effects to the compromised compartment and not the entire system. Unfortunately, the existing state-of-the-art embedded hardware-software solutions do not work well to enforce software compartmentalization for high-end embedded systems. MPUs are not fine-grained and suffer from significant scalability limitations as they can only protect a small and fixed number of memory regions. On the other hand, MMUs suffer from non-determinism and coarse-grained protection. This paper introduces CompartOS as a lightweight linkage-based compartmentalization model for high-end, complex, mainstream embedded systems. CompartOS builds on CHERI, a capability-based hardware architecture, to meet scalability, availability, compatibility, and fine-grained security goals. Microbenchmarks show that CompartOS' protection-domain crossing is 95% faster than MPU-based IPC. We applied the CompartOS model, with low effort, to complex existing systems, including TCP servers and a safety-critical automotive demo. CompartOS not only catches 10 out of 13 FreeRTOS-TCP published vulnerabilities that MPU-based protection (e.g., uVisor) cannot catch but can also recover from them. Further, our TCP throughput evaluations show that our CompartOS prototype is 52% faster than relevant MPU-based compartmentalization models (e.g., ACES), with a 15% overhead compared to an unprotected system. This comes at an FPGA's LUTs overhead of 10.4% to support CHERI for an unprotected baseline RISC-V processor, compared to 7.6% to support MPU, while CHERI only incurs 1.3% of the registers area overhead compared to 2% for MPU.

==> ipc_microbench_table.tex <==

\begin{table*}[t]
    \centering
    \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{l|ccccccccccccc}
            \toprule
            \multicolumn{1}{r}{}
            & \multicolumn{2}{c|}{CONTEXT\_SWITCH}
            & \multicolumn{2}{c|}{COMP\_FAULT}
            & \multicolumn{2}{c|}{FUNC\_CALL}
            & \multicolumn{2}{c|}{COMP\_CALL}
            & \multicolumn{2}{c|}{TASK\_NOTIFY}
            & \multicolumn{2}{c|}{TASK\_QUEUE} \\ \cline{2-13}
            & Instructions & Cycles & Instructions & Cycles & Instructions & Cycles & Instructions & Cycles & Instructions & Cycles & Instructions & Cycles & \\ \midrule
   \textbf{INSECURE-STATIC} & 177&475 & N/A&N/A & 8&118 & N/A&N/A & 495&2087 & 668&2433\\
\textbf{INSECURE-DYNAMIC} & 177&475 & N/A&N/A & 8&118 & N/A&N/A & 495&2212 & 668&2620\\
\textbf{PMP-4-TASKS} & 204&552 & N/A&N/A & 8&118 & N/A&N/A & 697&2585 & 867&3198\\
\textbf{PMP-16-OBJS} & 391&1246 & 409&1193 & 8&116 & 240&754 & 1053&3784 & 1223&4550\\
\textbf{PMP-N-OBJS} & 403&1270 & 589&1533 & 8&116 & 420&1151 & 1245&4327 & 1415&5006\\
\textbf{PMP-N-LIBS} & 368&917 & N/A&N/A & 8&116 & N/A&N/A & 1007&3580 & 1177&4136\\
\textbf{PURECAP} & 197&558 & N/A&N/A & 8&118 & N/A&N/A & 530&2244 & 753&2596\\
\textbf{COMPARTOS-LIBS} & 197&745 & N/A&N/A & 7&118 & N/A&N/A & 532&2604 & 759&3539\\
\textbf{COMPARTOS-OBJS} & 197&1002 & 230&1028 & 7&77 & 44&212 & 532&2778 & 759&3712\\

        \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{Number of instructions and cycles for microbenchmarks}
\label{table:microbench}
\end{table*}

